Cut Sparsification of the Clique Beyond the Ramanujan Bound: A Separation of Cut Versus Spectral Sparsification

We prove that a random $d$-regular graph, with high probability, is a cut sparsifier of the clique with approximation error at most $\left(2\sqrt{\frac 2 \pi} + o_{n,d}(1)\right)/\sqrt d$, where $2\sqrt{\frac 2 \pi} = 1.595\ldots$ and $o_{n,d}(1)$ denotes an error term that depends on $n$ and $d$ and goes to zero if we first take the limit $n\rightarrow \infty$ and then the limit $d \rightarrow \infty$. This is established by analyzing linear-size cuts using techniques of Jagannath and Sen derived from ideas in statistical physics, and analyzing small cuts via martingale inequalities. We also prove new lower bounds on spectral sparsification of the clique. If $G$ is a spectral sparsifier of the clique and $G$ has average degree $d$, we prove that the approximation error is at least the "Ramanujan bound'' $(2-o_{n,d}(1))/\sqrt d$, which is met by $d$-regular Ramanujan graphs, provided that either the weighted adjacency matrix of $G$ is a (multiple of) a doubly stochastic matrix, or that $G$ satisfies a certain high "odd pseudo-girth" property. The first case can be seen as an "Alon-Boppana theorem for symmetric doubly stochastic matrices," showing that a symmetric doubly stochastic matrix with $dn$ non-zero entries has a non-trivial eigenvalue of magnitude at least $(2-o_{n,d}(1))/\sqrt d$; the second case generalizes a lower bound of Srivastava and Trevisan, which requires a large girth assumption. Together, these results imply a separation between spectral sparsification and cut sparsification. If $G$ is a random $\log n$-regular graph on $n$ vertices, we show that, with high probability, $G$ admits a (weighted subgraph) cut sparsifier of average degree $d$ and approximation error at most $(1.595\ldots + o_{n,d}(1))/\sqrt d$, while every (weighted subgraph) spectral sparsifier of $G$ having average degree $d$ has approximation error at least $(2-o_{n,d}(1))/\sqrt d$.

==> conclusion.tex <==
\section{Concluding remarks}

We have demonstrated cut sparsification of the clique past the Ramanujan bound for spectral sparsification, and showed a separation between cut and spectral sparsification.

A matter of further interest is to extend the impossibility result for spectral sparsification to more general settings by relaxing or perhaps removing entirely the girth-related conditions of Theorem~\ref{th.lowerbound}. This could be done by designing a different pair of random walk vectors, which would remain nearly orthogonal to each other even in graphs that have short cycles.

It is natural then, to ask if the separation between cut and spectral sparsification extends to more general cases. Along these lines, it would be relevant to know if better cut sparsification results can be achieved for families of graphs beyond the complete graph.

The landscape of conceivable possibilities here is as yet wide open: for instance, it could possibly be the case that complete graphs are among the hardest graphs to spectrally sparsify, so that Theorem~\ref{th.lowerbound} in fact cannot be extended to graphs that require short cycles to spectrally sparsify.
On the other side, it could be that complete graphs are among the hardest to cut sparsify, and that we could in fact all graphs can be cut sparsified as well as or better than the clique.
A first step in that direction would be to demonstrate better cut sparsification than the twice-Ramanujan sparsifiers of Batson, Spielman and Srivastava \cite{BSS09} with sparsification of $2\sqrt{2}/\sqrt{d}$ for the worst-case graph.
The techniques we used to sparsify the complete graph are tailored to exploit large degrees of symmetry in the starting graph, however, and give little clue of how to extend to graphs without that symmetry.
Thus, generalizing the cut sparsification result will require new innovations.

